Fixing the functoriality of Khovanov homology: a simple approach

Khovanov homology is functorial up to sign with respect to link cobordisms. The sign indeterminacy has been fixed by several authors, by extending the original theory both conceptually and algebraically. In this paper we propose an alternative approach: we stay in the classical setup and fix the functoriality by simply adjusting the signs of the morphisms associated to the Reidemeister moves and the Morse moves.

==> corrections.tex <==
- The main proofs in the paper make use of c = v − u ̸= 0. This is correctly stated at the begin- ning of Sections 3 and 4. Since the results require c ̸= 0 while the original Khovanov homology corresponds to h = t = 0, and consequently c = 0, the paper does not fix the functoriality of the original Khovanov homology but rather that of the U (1) × U (1)-equivariant Khovanov-type homology. The author should change the title and the abstract to reflect this.

- For the same reason as above, the mention of the original Khovanov’s theory [Kho00] should be removed from the statement of Corollary 1.1.

- The assumption h2 + 4 ̸= 0 (which is equivalent to c ̸= 0) should be added to the assumption of Theorem 2. This is because the proof of the theorem relies on having c ̸= 0.

- page 2, line -6: Replace “then have BN(S)...” with “we have BN(S)...”

- Remark 3.2 should be given after Proposition 3.3, since it refers to the proof of Proposition 3.3. But I do not believe that the proof of Proposition 3.3 holds when c = 0, since the proof provided uses that the inclusion map ι satisfies ι(1) = c−1(a − b), which does not make sense when c = 0. In addition, when c = 0, the modified multiplication map is the zero map. I suggest that the author removes Remark 3.2.

- The author needs to refer to Figure 5. There is no reference or comment about this figure.

